TILDE-Q: A Transformation Invariant Loss Function for Time-Series Forecasting

Time-series forecasting has gained increasing attention in the field of artificial intelligence due to its potential to address real-world problems across various domains, including energy, weather, traffic, and economy. While time-series forecasting is a well-researched field, predicting complex temporal patterns such as sudden changes in sequential data still poses a challenge with current models. This difficulty stems from minimizing Lp norm distances as loss functions, such as mean absolute error (MAE) or mean square error (MSE), which are susceptible to both intricate temporal dynamics modeling and signal shape capturing. Furthermore, these functions often cause models to behave aberrantly and generate uncorrelated results with the original time-series. Consequently, developing a shape-aware loss function that goes beyond mere point-wise comparison is essential. In this paper, we examine the definition of shape and distortions, which are crucial for shape-awareness in time-series forecasting, and provide a design rationale for the shape-aware loss function. Based on our design rationale, we propose a novel, compact loss function called TILDEQ (Transformation Invariant Loss function with Distance EQuilibrium) that considers not only amplitude and phase distortions but also allows models to capture the shape of time-series sequences. Furthermore, TILDE-Q supports the simultaneous modeling of periodic and nonperiodic temporal dynamics. We evaluate the efficacy of TILDE-Q by conducting extensive experiments under both periodic and nonperiodic conditions with various models ranging from naive to state-of-the-art. The experimental results show that the models trained with TILDE-Q surpass those trained with other metrics, such as MSE and DILATE, in various real-world applications, including electricity, traffic, illness, economics, weather, and electricity transformer temperature (ETT).

==> table/NLinear_experiment.tex <==
\begin{table*}
\centering
\caption{Experimental results on Weather datasets (four cases) with NLinear.}
\begin{tabular}{c|c|cc|cc}
\toprule
\multicolumn{2}{c|}{Methods} & \multicolumn{2}{c|}{NLinear + MSE} & \multicolumn{2}{c}{NLinear + TILDE-Q} \\
\midrule
T   & IMP. & MSE    & LCSS   & MSE    & LCSS \\
\midrule\midrule
96  & +12.7\% & 0.0010 & 0.4378 & \textbf{0.0009} & \textbf{0.4802} \\
192 & +6.0\% & 0.0012 & 0.4087 & \textbf{0.0011} & \textbf{0.4370} \\
336 & +7.3\% & 0.0014 & 0.4034 & \textbf{0.0013} & \textbf{0.4189} \\
720 & +6.1\% & 0.0019 & 0.3870 & \textbf{0.0018} & \textbf{0.4009} \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}
\centering
\caption{Experimental results on Exchange datasets (four cases) with NLinear.}
\begin{tabular}{c|c|cc|cc}
\toprule
\multicolumn{2}{c|}{Methods} & \multicolumn{2}{c|}{NLinear + MSE} & \multicolumn{2}{c}{NLinear + TILDE-Q} \\
\midrule
T   & IMP. & MSE    & LCSS   & MSE    & LCSS \\
\midrule\midrule
96  & +2.1\% &  0.102 & 0.4352 & \textbf{0.100} & \textbf{0.4484} \\
192 & +5.2\% &  0.220 & 0.4339 & \textbf{0.210} & \textbf{0.4395} \\
336 & +3.9\% &  0.404 & 0.4105 & \textbf{0.389} & \textbf{0.4158} \\
720 & +0.0\% &  1.071 & 0.4020 & \textbf{1.070} & \textbf{0.4044} \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}
\centering
\caption{Experimental results on ETTh2 datasets (four cases) with NLinear.}
\begin{tabular}{c|c|cc|cc}
\toprule
\multicolumn{2}{c|}{Methods} & \multicolumn{2}{c|}{NLinear + MSE} & \multicolumn{2}{c}{NLinear + TILDE-Q} \\
\midrule
T   & IMP. & MSE    & LCSS   & MSE    & LCSS \\
\midrule\midrule
96  & -0.2\% & \textbf{0.129} & 0.6491 & 0.129 & \textbf{0.6618} \\
192 & +3.0\% & 0.169 & 0.6116 & \textbf{0.164} & \textbf{0.6285} \\
336 & +4.1\% & 0.194 & 0.5783 & \textbf{0.186} & \textbf{0.6118} \\
720 & +0.4\% & 0.225 & 0.5975 & \textbf{0.224} & \textbf{0.6020} \\
\bottomrule
\end{tabular}

\end{table*}

==> table/autoformer_experiment.tex <==

\begin{table*}[ht]
\centering
\caption{Detailed experimental results on six real-world datasets (four cases) with Autoformer.}
\resizebox{.95\columnwidth}{!}{\begin{tabular}{c|c|cccc|cccc|cccc}
\toprule
\multicolumn{2}{c|}{Methods} & \multicolumn{4}{c|}{Autoformer + MSE}& \multicolumn{4}{c|}{Autoformer + DILATE}& \multicolumn{4}{c}{Autoformer + \toolname}\\
\midrule
\multicolumn{2}{c|}{Metric}  & MSE         & DTW & TDI & LCSS & MSE         & DTW & TDI&LCSS & MSE         & DTW & TDI &LCSS\\
\midrule\midrule

 %GWNet - MemNet - Memnet(S) - MemNet+fourier - MemNet(S)+fourier - MemNet+free-emb - MemNet(S)+free-emb - MemNet(S)+free-emb + Euclidean
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTh2}}  
                                  &  96    & 0.1538 &  5.2227 &  2.1865 & 0.6187 & 0.2211 &  6.0453 &  2.5345 & 0.5315 & \textbf{0.1494} &  \textbf{5.1060} &  \textbf{1.9752} & \textbf{0.6317}\\
                                  & 192    & \textbf{0.1974} &  \textbf{7.8730} &  \textbf{3.3382} & \textbf{0.6019} & 0.2825 &  8.6696 &  5.6671 & 0.5335 & 0.2079 &  7.8917 &  3.7532 & 0.5984\\
                                  & 336    & 0.2393 & 10.8002 &  7.3141 & 0.5954 & 0.3759 & 11.0335 & 13.1347 & 0.5257 & \textbf{0.2360} & \textbf{10.7212} &  \textbf{7.0085} & \textbf{0.5971}\\
                                  & 720    & 0.2859 & 16.3502 & 15.9233 & 0.5772 & 0.4296 & 15.9819 & 22.2173 & 0.4924 & \textbf{0.2378} & \textbf{16.0002} & \textbf{13.7906} & \textbf{0.5795}\\
                                  \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTm2}}            
                                  &  96    & 0.0990 &  4.3498 &  2.5052 & 0.6756 & 0.1135 &  5.3097 &  \textbf{2.2211} & 0.5936 & \textbf{0.0940} &  \textbf{3.9078} & 2.2587 & \textbf{0.7075}\\
                                  & 192    & 0.1340 &  6.3207 &  3.3676 & 0.6512 & 0.1854 &  8.5209 &  3.7894 & 0.5506 & \textbf{0.1259} &  \textbf{6.0979} & \textbf{2.9278} & \textbf{0.6810}\\
                                  & 336    & 0.1587 &  \textbf{9.4374} &  6.9205 & 0.6036 & 0.2001 & 12.0265 &  8.8305 & 0.5370 & \textbf{0.1548} &  9.5223 & \textbf{7.2875} & \textbf{0.6169}\\
                                  & 720    & 0.1999 & 14.8332 & 11.9655 & 0.6064 & 0.2665 & 17.8025 & 17.4114 & 0.5001 & \textbf{0.1885} & \textbf{14.5844} & \textbf{9.9918} & \textbf{0.6277}\\
                                  \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ECL}}  
                                  &  96    & 0.4209 &  3.5957 & 0.2461 & 0.6487 & 0.6813 &  3.6490 & 0.4780 & 0.6253 & \textbf{0.3515} & \textbf{3.2173} & \textbf{0.2298} & \textbf{0.6912}\\
                                  & 192    & 0.4206 &  4.9924 & 0.3416 & 0.6574 & 0.7319 &  5.5324 & \textbf{0.2775} & 0.6118 & \textbf{0.4032} & \textbf{4.8581} & 0.3301 & \textbf{0.6680}\\
                                  & 336    & \textbf{0.4621} &  6.6888 & 0.2795 & \textbf{0.6535} & 0.7895 &  7.5665 & \textbf{0.2503} & 0.6091 & 0.4637 & \textbf{6.7335} & 0.3923 & 0.6429\\
                                  & 720    & \textbf{0.5005} & 10.8571 & 0.2383 & 0.6183 & 0.8630 & 12.1416 & \textbf{0.1877} & 0.6074 & 0.5049 & \textbf{9.8492} & 0.2525 & \textbf{0.6420}\\
                                  \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Exchange}}  
                                  &  96    & 0.2472 & 8.2957 & 5.8340 & 0.4577 & 0.1921 & 8.4651 & 5.6328 & \textbf{0.4646} & \textbf{0.1730} & \textbf{8.2046} & \textbf{5.1165} & 0.4577 \\
                                  & 192    & 0.3255 & 11.4212 & 17.0909 & 0.4319 & 0.4732 & 12.8599 & 19.0164 & 0.4124 & \textbf{0.2955} & \textbf{11.3655} & \textbf{15.4372} & \textbf{0.4433} \\
                                  & 336    & 0.5483 & \textbf{15.1853} & \textbf{44.4975} & 0.3277 & 0.8035 & 18.0948 & 57.5819 & 0.3114 & \textbf{0.5331} & 16.7350 & 45.8166 & \textbf{0.3321} \\
                                  & 720    & 1.3620 & 24.6397 & 145.3080 & \textbf{0.2357} & 1.4936 & 27.7069 & 151.6671 & 0.2302 & \textbf{1.1993} & \textbf{19.5296} & \textbf{121.8509} & 0.2233 \\
                                  \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Traffic}}            
                                  &  96    & 0.2562 & 1.9689 & 0.0178 & 0.8761 & 0.4835 & 1.9044 & 0.0392 & 0.8521 & \textbf{0.2275} & \textbf{1.8778} & \textbf{0.0168} & \textbf{0.8879} \\
                                  & 192    & 0.2604 & 2.8922 & \textbf{0.0091} & 0.8780 & 0.5653 & 3.0466 & 0.0343 & 0.8187 & \textbf{0.2497} & \textbf{2.8793} & 0.0116 & \textbf{0.8817} \\
                                  & 336    & 0.2474 & 4.0026 & \textbf{0.0051} & \textbf{0.8797} & 0.8155 & 4.2637 & 0.0327 & 0.8047 & \textbf{0.2422} & \textbf{3.9469} & 0.0059 & 0.8760 \\
                                  & 720    & \textbf{0.2720} & 6.4371 & \textbf{0.0030} & \textbf{0.8710} & 1.0729 & \textbf{6.0776} & 0.0217 & 0.8176 & 0.2836 & 6.1751 & 0.0034 & 0.8674 \\
                                  \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Weather}}  
                                  &  96    & 0.0168 &  7.4658 &  6.0336 & 0.4818 & 0.0019 &  \textbf{5.9775} &  4.9688 & 0.5306 & \textbf{0.0015} &  5.9829 &  \textbf{4.8957} & \textbf{0.5461} \\
                                  & 192    & 0.0069 & 10.6173 &  7.4506 & 0.4941 & 0.0026 &  8.3686 &  \textbf{5.4565} & \textbf{0.5423} & \textbf{0.0017} &  \textbf{7.7799} &  6.1032 & 0.5355 \\
                                  & 336    & 0.0052 & 12.5224 & 13.2607 & 0.4898 & 0.0030 & 12.4524 & 12.1816 & 0.4854 & \textbf{0.0020} & \textbf{10.3144} &  \textbf{9.0025} & \textbf{0.5252} \\
                                  & 720    & 0.0078 & 18.5079 & 25.8063 & 0.4744 & 0.0115 & 20.1354 & 36.7754 & 0.4721 & \textbf{0.0023} & \textbf{15.2563} & \textbf{18.3134} & \textbf{0.5102} \\
%\multicolumn{2}{c|}{Count}                 & 3     & 2 & 1 & 2 & 0 & 0 & 4 & 0 & 9 & 10 & 7 & 10\\
\bottomrule
\end{tabular}}
\label{tab:autoformer}
\end{table*}




==> table/fedformer_experiment.tex <==

\begin{table*}[ht]
\centering
\caption{Detailed experimental results on six real-world datasets (four cases) with FEDformer.}
\resizebox{.95\columnwidth}{!}{\begin{tabular}{c|c|cccc|cccc|cccc}
\toprule
\multicolumn{2}{c|}{Methods} & \multicolumn{4}{c|}{FEDformer + MSE}& \multicolumn{4}{c|}{FEDformer + DILATE}& \multicolumn{4}{c}{FEDformer + \toolname}\\
\midrule
\multicolumn{2}{c|}{Metric}  & MSE         & DTW & TDI & LCSS & MSE         & DTW & TDI&LCSS & MSE         & DTW & TDI &LCSS\\
\midrule\midrule

 %GWNet - MemNet - Memnet(S) - MemNet+fourier - MemNet(S)+fourier - MemNet+free-emb - MemNet(S)+free-emb - MemNet(S)+free-emb + Euclidean
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTh2}}  
                                  &  96    & \textbf{0.1299} &  \textbf{4.7265} &  \textbf{1.2607} & \textbf{0.6690} & 0.1906 &  6.2294 &  1.8228 & 0.5261 & 0.1381 &  4.7578 &  1.3560 & 0.6621 \\
                                  & 192    & \textbf{0.1819} &  7.6178 &  \textbf{2.6979} & \textbf{0.6229} & 0.2688 &  8.8422 &  4.8043 & 0.5261 & 0.1988 &  \textbf{7.6174} &  2.7712 & 0.6124 \\
                                  & 336    & \textbf{0.2305} & 10.5860 &  6.7027 & \textbf{0.6050} & 0.3506 & 11.4834 & 12.8408 & 0.5091 & 0.2382 & \textbf{10.4108} &  \textbf{6.6218} & 0.6039 \\
                                  & 720    & \textbf{0.2776} & 15.7013 & \textbf{14.7466} & \textbf{0.5911} & 0.4327 & \textbf{14.0692} & 20.6266 & 0.5091 & 0.2871 & 15.3120 & 16.4059 & 0.5808 \\
                                  \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTm2}}            
                                  &  96    & 0.0682 &  3.0962 &  1.3862 & 0.7868 & 0.1147 &  4.6648 &  2.2981 & 0.6325 & \textbf{0.0669} &  \textbf{3.0328} &  \textbf{1.3556} & \textbf{0.7918} \\
                                  & 192    & 0.0976 &  5.2417 &  \textbf{2.0295} & 0.7340 & 0.1848 &  8.0678 &  4.4893 & 0.5391 & \textbf{0.0971} &  \textbf{5.1508} &  2.1782 & \textbf{0.7384} \\
                                  & 336    & 0.1326 &  8.3151 &  5.4619 & 0.6667 & 0.2493 & 13.6349 & 11.7563 & 0.5049 & \textbf{0.1279} &  \textbf{8.3010} &  \textbf{4.5488} & \textbf{0.6828} \\
                                  & 720    & 0.1957 & 14.2579 & 11.8328 & 0.6262 & 0.2913 & 17.4636 & 41.9434 & 0.4806 & \textbf{0.1822} & \textbf{14.1131} & \textbf{10.4778} & \textbf{0.6361} \\
                                  \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ECL}}  
                                  &  96    & \textbf{0.2531} &  \textbf{2.6402} & \textbf{0.1436} & \textbf{0.7322} & 0.4794 &  2.8685 & 0.2482 & 0.6943 & 0.2638 &  2.6594 & 0.1614 & 0.7265 \\
                                  & 192    & 0.2945 &  3.8647 & 0.1831 & 0.7306 & 0.5485 &  4.3313 & 0.1732 & 0.6813 & \textbf{0.2821} &  \textbf{3.7830} & \textbf{0.1277} & \textbf{0.7340} \\
                                  & 336    & \textbf{0.3313} &  5.2789 & \textbf{0.1078} & 0.7207 & 0.6967 &  5.7911 & 0.1985 & 0.6892 & 0.3385 &  \textbf{5.1763} & 0.1229 & \textbf{0.7290} \\
                                  & 720    & 0.3956 &  8.5881 & \textbf{0.0632} & 0.6961 & 0.7741 & 10.1163 & 0.8837 & 0.6403 & \textbf{0.3939} &  \textbf{8.5665} & 0.0784 & \textbf{0.7013} \\
                                  \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Exchange}}  
                                  &  96    & 0.1437 &  8.5595 &   \textbf{4.4258} & 0.4347 & 0.3884 &  8.9178 &   7.0385 & 0.4439 & \textbf{0.1215} &  \textbf{8.0591} &   6.1979 & \textbf{0.4704} \\
                                  & 192    & \textbf{0.2694} & 12.5168 &  12.3117 & 0.4202 & 0.5912 & 13.1929 &  15.4207 & 0.4187 & 0.2956 & \textbf{11.5607} &  \textbf{12.1302} & \textbf{0.4474} \\
                                  & 336    & \textbf{0.4916} & 16.4673 &  27.0756 & 0.4140 & 0.7520 & 18.1381 &  33.7878 & 0.3969 & 0.5896 & \textbf{15.9267} &  \textbf{24.8808} & \textbf{0.4342} \\
                                  & 720    & 1.2115 & 25.6243 & 108.0500 & 0.3838 & 1.5110 & 26.7031 &  91.6313 & 0.3760 & \textbf{1.1700} & \textbf{24.6190} &  \textbf{71.8783} & \textbf{0.3935} \\
                                  \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Traffic}}            
                                  &  96    & 0.2074 & 1.9132 & 0.0165 & 0.8824 & 0.3533 & 1.8617 & 0.0291 & 0.8609 & \textbf{0.1867} & \textbf{1.8386} & \textbf{0.0152} & \textbf{0.8983} \\
                                  & 192    & 0.2051 & 2.7761 & 0.0085 & 0.8951 & 1.4682 & 2.7545 & 0.1312 & 0.8591 & \textbf{0.1961} & \textbf{2.7380} & \textbf{0.0083} & \textbf{0.8975} \\
                                  & 336    & 0.2140 & \textbf{3.7583} & \textbf{0.0047} & \textbf{0.9023} & 2.9741 & 3.7440 & 0.1779 & 0.8519 & \textbf{0.2059} & 3.7834 & 0.0050 & 0.8947 \\
                                  & 720    & \textbf{0.2291} & \textbf{5.9735} & 0.0026 & \textbf{0.8919} & 3.0829 & 5.8173 & 0.0949 & 0.8580 & 0.2312 & 6.1080 & \textbf{0.0022} & 0.8735 \\
                                  \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Weather}}  
                                  &  96    & 0.0070 &  6.1550 &  4.7039 & 0.5264 & 0.0017 &  5.9507 &  4.5891 & 0.5535 & \textbf{0.0014} &  \textbf{5.5205} &  \textbf{4.1085} & \textbf{0.5792} \\
                                  & 192    & 0.0063 &  7.6906 &  6.2940 & 0.5417 & 0.0020 &  8.6593 &  \textbf{4.6333} & \textbf{0.6000} & \textbf{0.0017} &  \textbf{6.9706} &  5.0003 & 0.5863 \\
                                  & 336    & 0.0046 & 10.3501 &  9.4691 & 0.5261 & 0.0053 & 14.8249 &  9.6239 & 0.4801 & \textbf{0.0018} &  \textbf{9.3016} &  \textbf{7.4610} & \textbf{0.5784} \\
                                  & 720    & 0.0060 & 15.2429 & 24.5379 & 0.4911 &      0.0029 &       16.3929 &       20.0782 &      0.4892 & \textbf{0.0024} & \textbf{13.7936} & \textbf{15.7668} & \textbf{0.5737} \\
%\multicolumn{2}{c|}{Count}                 & 3     & 2 & 1 & 2 & 0 & 0 & 4 & 0 & 9 & 10 & 7 & 10\\
\bottomrule
\end{tabular}}
\label{tab:fedformer}
\end{table*}



\iffalse
% ± ([0-9]+.[0-9]+)
asdf









\fi


==> table/informer_experiment.tex <==
\begin{table*}[ht]
\centering
\caption{Detailed experimental results on six real-world datasets (four cases) with Informer.}
\resizebox{.95\columnwidth}{!}{\begin{tabular}{c|c|cccc|cccc|cccc}
\toprule
\multicolumn{2}{c|}{Methods} & \multicolumn{4}{c|}{Informer + MSE}& \multicolumn{4}{c|}{Informer + DILATE}& \multicolumn{4}{c}{Informer + \toolname}\\
\midrule
\multicolumn{2}{c|}{Metric}  & MSE         & DTW & TDI & LCSS & MSE         & DTW & TDI&LCSS & MSE         & DTW & TDI &LCSS\\
\midrule\midrule

 %GWNet - MemNet - Memnet(S) - MemNet+fourier - MemNet(S)+fourier - MemNet+free-emb - MemNet(S)+free-emb - MemNet(S)+free-emb + Euclidean
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTh2}}  
                                  &  96    &0.2466 &  6.9254 &  3.6676 & 0.4633 & 0.3284 &  6.3109 &  3.5838 & 0.5037 & \textbf{0.1768} &  \textbf{5.8437} &  \textbf{1.6734} & \textbf{0.5379}\\
                                  & 192    &0.2818 & 10.2654 & 11.1580 & 0.4254 & 0.4086 &  \textbf{8.8262} &  \textbf{7.1780} & \textbf{0.4893} & \textbf{0.2432} & 10.2134 &  9.9865 & 0.4317\\
                                  & 336    &0.3089 & 12.1822 & 18.7014 & 0.4434 & 0.4164 & \textbf{10.3779} & \textbf{13.2580} & \textbf{0.5062} & \textbf{0.2958} & 13.5586 & 20.2850 & 0.4165\\
                                  & 720    &\textbf{0.2877} & 17.6369 & 38.4617 & 0.4425 & 0.4229 & \textbf{14.1196} & \textbf{23.9403} & \textbf{0.4815} & 0.3157 & 18.4617 & 43.3238 & 0.4262\\
                                  \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTm2}}            
                                  &  96    &0.0889 &  3.4007 &  1.5719 & 0.7386 & 0.1263 &  6.0144 &  2.7757 & 0.5129 & \textbf{0.0871} &  \textbf{3.1354} &  \textbf{1.3474} & \textbf{0.7817}\\
                                  & 192    &\textbf{0.1157} &  5.7964 &  \textbf{2.8128} & 0.6705 & 0.2340 &  9.7004 &  7.8354 & 0.5266 & 0.1317 &  \textbf{5.7093} &  2.9129 & \textbf{0.6983}\\
                                  & 336    &0.1860 &  \textbf{8.9971} &  \textbf{6.7970} & 0.6365 & 0.2805 & 11.7889 & 13.3861 & 0.5025 & \textbf{0.1767} &  9.0866 &  7.4023 & \textbf{0.6555}\\
                                  & 720    &0.2165 & 14.7685 & 24.6694 & 0.5768 & 0.3745 & 16.7734 & 29.2783 & 0.4747 & \textbf{0.2063} & \textbf{15.3057} & \textbf{24.1959} & \textbf{0.5860}\\
                                  \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ECL}}  
                                  &  96    &\textbf{0.2709} &  \textbf{2.8067} & \textbf{0.1720} & 0.7032 & 0.9856 &  3.6394 & 1.4794 & 0.6324 & 0.2800 &  2.9466 & 0.2473 & \textbf{0.7275}\\
                                  & 192    &\textbf{0.2793} &  \textbf{4.1193} & \textbf{0.1508} & 0.7060 & 1.1209 &  5.2289 & 2.1749 & 0.6053 & 0.3077 &  4.2693 & 0.2978 & \textbf{0.7336}\\
                                  & 336    &0.3203 &  5.9533 & 0.1642 & 0.7222 & 1.2331 &  7.8470 & 3.0415 & 0.5694 & \textbf{0.3271} &  \textbf{5.8090} & \textbf{0.1984} & \textbf{0.7143}\\
                                  & 720    &0.6414 & 15.8561 & 4.4284 & 0.4564 & 1.3706 & 12.5981 & 5.6720 & 0.5506 & \textbf{0.4676} & \textbf{11.4027} & \textbf{0.7107} & \textbf{0.6298}\\
                                  %\midrule
                                  \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Exchange}}  
                                  &  96    & 0.3534 &  8.0965 &  \textbf{4.8843} & \textbf{0.4689} & \textbf{0.3260} & \textbf{7.7370} &  5.6336 & 0.4678 & 0.5264 &  7.9866 &  6.5120 & 0.4553 \\
                                  & 192    & \textbf{0.9682} & 11.0843 & 11.3110 & 0.4647 & 0.9737 & 10.8894 & 15.6770 & 0.4584 & 1.2845 & \textbf{10.4358} & \textbf{10.7009} & \textbf{0.4959} \\
                                  & 336    & \textbf{1.3710} & 12.8076 & 18.5937 & 0.4676 & 1.6735 & 12.7034 & 29.2013 & 0.4428 & 1.6912 & \textbf{12.2349} & \textbf{18.2197} & \textbf{0.4932} \\
                                  & 720    & \textbf{1.7586} & 22.6852 & 59.4243 & 0.4681 & 1.8292 & \textbf{16.0093} & \textbf{56.8687} & \textbf{0.5293} & 1.9130 & 24.0510 & 62.8152 & 0.5104 \\
                                  \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Traffic}}            
                                  &  96    & 0.2606 &  2.0994 & 0.0208 & 0.8329 & 2.9612 &  2.3355 & 0.9646 & 0.7312 & \textbf{0.2284} &  \textbf{2.0027} & \textbf{0.0194} & \textbf{0.8490} \\
                                  & 192    & 0.2920 &  3.2573 & 0.0126 & 0.8158 & 2.9978 &  3.5451 & 0.8429 & 0.7394 & \textbf{0.2753} &  \textbf{3.1721} & \textbf{0.0125} & \textbf{0.8248} \\
                                  & 336    & 0.3109 &  4.6581 & 0.0078 & 0.8115 & 2.9696 &  4.9879 & 1.2672 & 0.7117 & \textbf{0.2993} &  \textbf{4.4715} & \textbf{0.0077} & \textbf{0.8170} \\
                                  & 720    & \textbf{0.3472} &  \textbf{6.7989} & \textbf{0.0040} & \textbf{0.8146} & 2.6845 & 10.7450 & 3.4514 & 0.5874 & 0.3859 &  7.5424 & 0.0051 & 0.7752 \\
                                  \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Weather}}  
                                  &  96    & 0.0043 &  8.2890 &  5.4604 & 0.4556 & 0.0069 &  6.5571 &  4.7505 & 0.5159 & \textbf{0.0021} &  \textbf{5.5412} &  \textbf{4.5012} & \textbf{0.5602} \\
                                  & 192    & 0.0031 & 10.7993 &  9.2928 & 0.4523 & 0.0041 & 10.5645 &  9.4713 & 0.4704 & \textbf{0.0028} &  \textbf{8.2535} &  \textbf{5.8289} & \textbf{0.5516} \\
                                  & 336    & 0.0051 & 13.8721 & 22.2699 & 0.4451 & 0.0055 & 12.0586 & 16.4933 & 0.4884 & \textbf{0.0039} & \textbf{10.8802} & \textbf{10.5220} & \textbf{0.5668} \\
                                  & 720    & 0.0061 & 21.7720 & 41.5877 & 0.4476 & 0.0737 & 16.8378 & 29.8112 & 0.5142 & \textbf{0.0047} & \textbf{13.9934} & \textbf{20.9991} & \textbf{0.5689} \\
%\multicolumn{2}{c|}{Count}                 & 4     & 3 & 4 & 0 & 0 & 3 & 3 & 3 & 8 & 6 & 5 & 9\\
\bottomrule
\end{tabular}}
\label{tab:informer}
\end{table*}

\iffalse
% ± ([0-9]+.[0-9]+)
asdf



\fi

==> table/main_table.tex <==


%Table 순서 - NBeats, Informer, Autoformer, FEDformer
% Data 순서 - ETTh2, ETTm2, ECL, Exchange, Traffic, Weather

\setlength{\tabcolsep}{3.5pt}
\begin{table*}
\centering
\caption{Experimental results on six real-world datasets (four cases) with four the state-of-the-art models and three training metrics. For all experiment, we set input sequence length $T = 96$.}
\resizebox{.95\columnwidth}{!}{
\begin{tabular}{c|c|cc|cc|cc||cc|cc|cc||cc|cc|cc||cc|cc|cc} 
\toprule
\multicolumn{2}{c|}{Model} & \multicolumn{6}{c||}{N-Beats} & \multicolumn{6}{c||}{Informer} & \multicolumn{6}{c||}{Autoformer} & \multicolumn{6}{c}{FEDformer} \\
\midrule
\multicolumn{2}{c|}{Methods} & \multicolumn{2}{c|}{MSE} & \multicolumn{2}{c|}{DILATE} & \multicolumn{2}{c||}{TILDE-Q} & \multicolumn{2}{c|}{MSE} & \multicolumn{2}{c|}{DILATE} & \multicolumn{2}{c||}{TILDE-Q} & \multicolumn{2}{c|}{MSE} & \multicolumn{2}{c|}{DILATE} & \multicolumn{2}{c||}{TILDE-Q} & \multicolumn{2}{c|}{MSE} & \multicolumn{2}{c|}{DILATE} & \multicolumn{2}{c}{TILDE-Q} \\
\midrule
 \multicolumn{2}{c|}{Metric}                                      & MSE   & LCSS  & MSE   & LCSS  & MSE   & LCSS & MSE   & LCSS  & MSE   & LCSS  & MSE   & LCSS  & MSE   & LCSS  & MSE   & LCSS  & MSE   & LCSS  & MSE   & LCSS  & MSE   & LCSS  & MSE   & LCSS  \\ 
\midrule[\heavyrulewidth]
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTh2}}            & 96  & 0.187 & 0.468 & 0.310 & 0.487 & \textbf{0.155} & \textbf{0.586} & 0.246 & 0.463 & 0.328 & 0.503 & \textbf{0.176} & \textbf{0.537} & 0.153 & 0.618 & 0.221 & 0.531 & \textbf{0.149} & \textbf{0.631} & \textbf{0.130} & \textbf{0.669} & 0.191 & 0.526 & 0.138 & 0.662 \\
                                                            & 192 & 0.239 & 0.450 & 0.618 & 0.463 & \textbf{0.173} & \textbf{0.581} & 0.281 & 0.425 & 0.408 & \textbf{0.489} & \textbf{0.243} & 0.431 & \textbf{0.197} & \textbf{0.601} & 0.282 & 0.533 & 0.207 & 0.598 & \textbf{0.182} & \textbf{0.623} & 0.269 & 0.526 & 0.199 & 0.612 \\
                                                            & 336 & 0.289 & 0.454 & 1.140 & 0.458 & \textbf{0.213} & \textbf{0.537} & 0.308 & 0.443 & 0.416 & \textbf{0.506} & \textbf{0.295} & 0.416 & 0.239 & 0.595 & 0.375 & 0.525 & \textbf{0.236} & \textbf{0.597} & \textbf{0.230} & \textbf{0.605} & 0.351 & 0.509 & 0.238 & 0.604 \\
                                                            & 720 & 0.388 & 0.438 & 1.671 & 0.457 & \textbf{0.304} & \textbf{0.528} & \textbf{0.287} & 0.442 & 0.422 & \textbf{0.481} & 0.315 & 0.426 & 0.285 & 0.577 & 0.429 & 0.492 & \textbf{0.237} & \textbf{0.579} & \textbf{0.278} & \textbf{0.591} & 0.433 & 0.509 & 0.287 & 0.581 \\ 
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTm2}}            & 96  & \textbf{0.079} & 0.672 & 0.152 & 0.437 & 0.095 & \textbf{0.690} & 0.088 & 0.738 & 0.126 & 0.512 & \textbf{0.087} & \textbf{0.781} & 0.099 & 0.675 & 0.113 & 0.593 & \textbf{0.094} & \textbf{0.707} & 0.068 & 0.787 & 0.115 & 0.632 & \textbf{0.067} & \textbf{0.792} \\
                                                            & 192 & \textbf{0.122} & 0.576 & 0.205 & 0.510 & 0.128 & \textbf{0.616} & \textbf{0.115} & 0.670 & 0.234 & 0.526 & 0.131 & \textbf{0.698} & 0.134 & 0.651 & 0.185 & 0.550 & \textbf{0.125} & \textbf{0.681} & 0.098 & 0.734 & 0.185 & 0.539 & \textbf{0.097} & \textbf{0.738} \\
                                                            & 336 & 0.182 & 0.458 & 0.250 & 0.481 & \textbf{0.170} & \textbf{0.619} & 0.186 & 0.636 & 0.280 & 0.502 & \textbf{0.176} & \textbf{0.655} & 0.158 & 0.603 & 0.200 & 0.537 & \textbf{0.154} & \textbf{0.616} & 0.133 & 0.667 & 0.249 & 0.505 & \textbf{0.127} & \textbf{0.682} \\
                                                            & 720 & 0.237 & 0.492 & 0.417 & 0.583 & \textbf{0.233} & \textbf{0.707} & 0.216 & 0.576 & 0.374 & 0.474 & \textbf{0.206} & \textbf{0.586} & 0.199 & 0.606 & 0.266 & 0.500 & \textbf{0.188} & \textbf{0.627} & 0.196 & 0.626 & 0.291 & 0.481 & \textbf{0.182} & \textbf{0.636} \\ 
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ECL}}              & 96  & 0.366 & 0.658 & 1.115 & 0.507 & \textbf{0.318} & \textbf{0.722} & \textbf{0.270} & 0.703 & 0.985 & 0.632 & 0.280 & \textbf{0.727} & 0.420 & 0.648 & 0.681 & 0.625 & \textbf{0.351} & \textbf{0.691} & \textbf{0.253} & \textbf{0.732} & 0.479 & 0.694 & 0.264 & 0.727 \\
                                                            & 192 & 0.430 & 0.621 & 1.185 & 0.497 & \textbf{0.338} & \textbf{0.718} & \textbf{0.279} & 0.706 & 1.120 & 0.605 & 0.307 & \textbf{0.733} & 0.420 & 0.657 & 0.731 & 0.611 & \textbf{0.403} & \textbf{0.668} & 0.295 & 0.731 & 0.549 & 0.681 & \textbf{0.282} & \textbf{0.734} \\
                                                            & 336 & 0.519 & 0.596 & 1.246 & 0.509 & \textbf{0.383} & \textbf{0.711} & \textbf{0.320} & \textbf{0.722} & 1.233 & 0.569 & 0.327 & 0.714 & \textbf{0.462} & \textbf{0.653} & 0.789 & 0.609 & 0.463 & 0.642 & \textbf{0.331} & 0.721 & 0.697 & 0.689 & 0.339 & \textbf{0.730} \\
                                                            & 720 & 0.624 & 0.571 & 1.306 & 0.533 & \textbf{0.454} & \textbf{0.696} & 0.641 & 0.456 & 1.370 & 0.550 & \textbf{0.467} & \textbf{0.629} & \textbf{0.500} & 0.618 & 0.863 & 0.607 & 0.504 & \textbf{0.642} & 0.396 & 0.696 & 0.774 & 0.640 & \textbf{0.394} & \textbf{0.701} \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Exchange}}         & 96  & 0.450 & 0.442 & 0.394 & 0.432 & \textbf{0.275} & \textbf{0.447} & 0.353 & \textbf{0.469} & \textbf{0.326} & 0.468 & 0.526 & 0.455 & 0.247 & 0.458 & 0.192 & \textbf{0.465} & \textbf{0.173} & 0.458 & 0.144 & 0.435 & 0.388 & 0.444 & \textbf{0.122} & \textbf{0.470} \\
                                                            & 192 & \textbf{1.216} & 0.416 & 1.568 & 0.406 & 1.662 & \textbf{0.435} & \textbf{0.968} & 0.465 & 0.974 & 0.458 & 1.285 & \textbf{0.496} & 0.325 & 0.432 & 0.473 & 0.412 & \textbf{0.295} & \textbf{0.443} & \textbf{0.269} & 0.420 & 0.591 & 0.419 & 0.296 & \textbf{0.447} \\
                                                            & 336 & \textbf{1.453} & 0.413 & 3.678 & 0.387 & 1.843 & \textbf{0.460} & \textbf{1.371} & 0.468 & 1.673 & 0.443 & 1.691 & \textbf{0.493} & 0.548 & 0.328 & 0.803 & 0.311 & \textbf{0.533} & \textbf{0.332} & \textbf{0.492} & 0.414 & 0.752 & 0.397 & 0.590 & \textbf{0.434} \\
                                                            & 720 & \textbf{1.856} & 0.407 & 3.901 & 0.340 & 2.849 & \textbf{0.462} & \textbf{1.764} & 0.468 & 1.829 & \textbf{0.529} & 1.913 & 0.510 & 1.362 & \textbf{0.236} & 1.494 & 0.230 & \textbf{1.199} & 0.223 & 1.212 & 0.384 & 1.511 & 0.376 & \textbf{1.170} & \textbf{0.393} \\ 
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Traffic}}          & 96  & 0.234 & 0.830 & 2.332 & 0.525 & \textbf{0.229} & \textbf{0.837} & 0.261 & 0.833 & 2.961 & 0.731 & \textbf{0.228} & \textbf{0.849} & 0.256 & 0.876 & 0.483 & 0.852 & \textbf{0.227} & \textbf{0.888} & 0.207 & 0.882 & 0.353 & 0.861 & \textbf{0.187} & \textbf{0.898} \\
                                                            & 192 & \textbf{0.301} & 0.792 & 2.563 & 0.552 & 0.335 & \textbf{0.803} & 0.292 & 0.816 & 2.998 & 0.739 & \textbf{0.275} & \textbf{0.825} & 0.260 & 0.878 & 0.565 & 0.819 & \textbf{0.250} & \textbf{0.882} & 0.205 & 0.895 & 1.468 & 0.859 & \textbf{0.196} & \textbf{0.898} \\
                                                            & 336 & \textbf{0.345} & 0.792 & 2.460 & 0.521 & 0.399 & \textbf{0.821} & 0.311 & 0.811 & 2.970 & 0.712 & \textbf{0.299} & \textbf{0.817} & 0.247 & \textbf{0.880} & 0.816 & 0.805 & \textbf{0.242} & 0.876 & 0.214 & \textbf{0.902} & 2.974 & 0.852 & \textbf{0.206} & 0.895 \\
                                                            & 720 & \textbf{0.430} & 0.796 & 2.352 & 0.518 & 0.448 & \textbf{0.809} & \textbf{0.347} & \textbf{0.815} & 2.685 & 0.587 & 0.386 & 0.775 & \textbf{0.272} & \textbf{0.871} & 1.073 & 0.818 & 0.284 & 0.868 & \textbf{0.229} & \textbf{0.892} & 3.083 & 0.858 & 0.231 & 0.873 \\ 
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Weather}}          & 96  & 0.004 & 0.407 & 0.002 & 0.426 & \textbf{0.001} & \textbf{0.517} & 0.004 & 0.456 & 0.007 & 0.516 & \textbf{0.002} & \textbf{0.560} & 0.017 & 0.482 & 0.002 & 0.531 & \textbf{0.001} & \textbf{0.546} & 0.007 & 0.526 & 0.002 & 0.554 & \textbf{0.001} & \textbf{0.579} \\
                                                            & 192 & 0.006 & 0.421 & 0.003 & 0.431 & \textbf{0.002} & \textbf{0.508} & 0.003 & 0.452 & 0.004 & 0.470 & \textbf{0.003} & \textbf{0.552} & 0.007 & 0.494 & 0.003 & \textbf{0.542} & \textbf{0.002} & 0.535 & 0.006 & 0.542 & 0.003 & \textbf{0.600} & \textbf{0.002} & 0.586 \\
                                                            & 336 & 0.006 & 0.424 & 0.009 & 0.358 & \textbf{0.003} & \textbf{0.507} & 0.005 & 0.445 & 0.005 & 0.488 & \textbf{0.004} & \textbf{0.567} & 0.005 & 0.490 & 0.003 & 0.485 & \textbf{0.002} & \textbf{0.525} & 0.005 & 0.526 & 0.005 & 0.480 & \textbf{0.002} & \textbf{0.578} \\
                                                            & 720 & 0.007 & 0.432 & 0.153 & 0.398 & \textbf{0.003} & \textbf{0.508} & 0.006 & 0.448 & 0.074 & 0.514 & \textbf{0.005} & \textbf{0.569} & 0.008 & 0.474 & 0.011 & 0.472 & \textbf{0.002} & \textbf{0.510} & 0.006 & 0.491 &     0.003 &     0.489 & \textbf{0.002} & \textbf{0.574} \\
%\midrule[\heavyrulewidth]
%\multicolumn{2}{c|}{Count} & 8 & 0 & 0 & 0 & \textbf{16} & \textbf{24} & 9 & 3 & 1 & 4 & \textbf{14} & \textbf{17} & 4 & 4 & 0 & 1 & \textbf{20} & \textbf{17} & 9 & 7 & 0 & 1 & \textbf{15} & \textbf{16} \\
\bottomrule
\end{tabular}
}
\label{tab:main_results}
\end{table*}



==> table/nbeats_experiment.tex <==

\begin{table*}[ht]
\centering
\caption{Detailed experimental results on six real-world datasets (four cases) with N-Beats.}
\resizebox{.95\columnwidth}{!}{\begin{tabular}{c|c|cccc|cccc|cccc}
\toprule
\multicolumn{2}{c|}{Methods} & \multicolumn{4}{c|}{N-Beats + MSE}& \multicolumn{4}{c|}{N-Beats + DILATE}& \multicolumn{4}{c}{N-Beats + \toolname}\\
\midrule
\multicolumn{2}{c|}{Metric}  & MSE         & DTW & TDI & LCSS & MSE         & DTW & TDI&LCSS & MSE         & DTW & TDI &LCSS\\
\midrule\midrule 

 %GWNet - MemNet - Memnet(S) - MemNet+fourier - MemNet(S)+fourier - MemNet+free-emb - MemNet(S)+free-emb - MemNet(S)+free-emb + Euclidean
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTh2}}  
                                  &  96    & 0.1869 &  7.2379 &  2.3787 & 0.4688 & 0.3105 &  6.5849 &  3.6490 & 0.4879 & \textbf{0.1557} &  \textbf{5.1011} & \textbf{1.3240} & \textbf{0.5862}\\
                                  & 192    & 0.2385 & 11.5667 &  4.9153 & 0.4505 & 0.6186 &  9.7254 &  7.0831 & 0.4637 & \textbf{0.1738} &  \textbf{7.6334} & \textbf{2.4122} & \textbf{0.5819}\\
                                  & 336    & 0.2889 & 16.5255 & 11.5207 & 0.4544 & 1.1406 & 13.7328 & 14.6986 & 0.4584 & \textbf{0.2132} & \textbf{11.3351} & \textbf{5.3556} & \textbf{0.5373}\\
                                  & 720    & 0.3881 & 24.1570 & 18.8462 & 0.4381 & 1.6713 & 19.4392 & 23.7028 & 0.4575 & \textbf{0.3044} & \textbf{17.6006} & \textbf{9.6636} & \textbf{0.5287}\\
                                  \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTm2}}            
                                  &  96    & \textbf{0.0790} &  \textbf{3.9685} &  \textbf{2.0436} & 0.6721 & 0.1524 &  7.9302 &  5.5597 & 0.4379 & 0.0952 &  4.0110 &  2.1939 & \textbf{0.6902}\\
                                  & 192    & \textbf{0.1224} &  6.8695 &  \textbf{3.2834} & 0.5762 & 0.2055 & 10.0393 &  8.5602 & 0.5107 & 0.1286 &  \textbf{6.3556} &  4.9798 & \textbf{0.6160}\\
                                  & 336    & 0.1824 & 12.1438 &  8.5915 & 0.4587 & 0.2501 & 12.6342 & 16.1473 & 0.4819 & \textbf{0.1705} &  \textbf{8.9377} &  \textbf{8.3539} & \textbf{0.6195}\\
                                  & 720    & 0.2370 & 22.8676 & 17.8458 & 0.4929 & 0.4170 & 17.7764 & 24.6877 & 0.5836 & \textbf{0.2336} & \textbf{14.2715} & \textbf{19.0883} & \textbf{0.7070}\\
                                  \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ECL}}  
                                  &  96    & 0.3666 &  3.5207 & 0.2989 & 0.6589 & 1.1156 &  5.1430 & 2.6613 & 0.5074 & \textbf{0.3183} & \textbf{2.9707} & \textbf{0.4844} & \textbf{0.7229}\\
                                  & 192    & 0.4307 &  5.7578 & 0.4253 & 0.6212 & 1.1859 &  7.3406 & 2.8488 & 0.4973 & \textbf{0.3383} & \textbf{4.1817} & \textbf{0.4229} & \textbf{0.7187}\\
                                  & 336    & 0.5199 &  8.5563 & 0.5384 & 0.5965 & 1.2460 &  9.5096 & 3.0517 & 0.5091 & \textbf{0.3831} & \textbf{5.6643} & \textbf{0.3024} & \textbf{0.7112}\\
                                  & 720    & 0.6240 & 13.9436 & 0.6510 & 0.5717 & 1.3061 & 13.1928 & 3.7279 & 0.5337 & \textbf{0.4540} & \textbf{8.9997} & \textbf{0.3251} & \textbf{0.6960}\\
                                  \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Exchange}}  
                                  &  96    & 0.4496 &  8.6395 &  \textbf{4.3197} & 0.4424 & 0.3945 &  8.9661 &  4.3286 & 0.4316 & \textbf{0.2748} &  \textbf{7.9744} &  5.2964 & \textbf{0.4467} \\
                                  & 192    & \textbf{1.2161} & 12.1857 & 10.5166 & 0.4157 & 1.5684 & 13.0560 &  9.2434 & 0.4061 & 1.6629 & \textbf{11.5557} &  \textbf{8.7896} & \textbf{0.4348} \\
                                  & 336    & \textbf{1.4529} & 14.7085 & 19.0407 & 0.4130 & 3.6784 & 17.5189 & \textbf{17.2512} & 0.3871 & 1.8432 & \textbf{12.5648} & 20.8871 & \textbf{0.4603} \\
                                  & 720    & \textbf{1.8563} & 21.7347 & \textbf{50.6751} & 0.4073 & 3.9008 & 26.7020 & 74.0546 & 0.3400 & 2.8487 & \textbf{19.1588} & 53.8069 & \textbf{0.4619} \\
                                  \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Traffic}}            
                                  &  96    & 0.2349 & 2.1046 & 0.0216 & 0.8303 & 2.3325 & 3.9657 &  1.2052 & 0.5250 & \textbf{0.2286} & \textbf{2.0699} & \textbf{0.0207} & \textbf{0.8371} \\
                                  & 192    & \textbf{0.3014} & 3.4040 & 0.0142 & 0.7916 & 2.5627 &  5.4169 & 1.1355 & 0.5515 & 0.3352 & \textbf{3.2559} & \textbf{0.0119} & \textbf{0.8028} \\
                                  & 336    & \textbf{0.3455} & 4.6409 & 0.0088 & 0.7918 & 2.4599 &  8.2828 & 1.3377 & 0.5208 & 0.3990 & \textbf{4.2622} & \textbf{0.0066} & \textbf{0.8206} \\
                                  & 720    & \textbf{0.4298} & 7.0561 & 0.0045 & 0.7958 & 2.3522 & 12.6258 & 0.9967 & 0.5177 & 0.4480 & \textbf{6.7344} & \textbf{0.0034} & \textbf{0.8085} \\
                                  \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Weather}}  
                                  &  96    & 0.0042 & 9.3228 & 5.9134 & 0.4072 & 0.0023 & 8.9289 & \textbf{5.0617} & 0.4256 & \textbf{0.0010} & \textbf{6.5198} & 6.0450 & \textbf{0.5168} \\
                                  & 192    & 0.0056 & 10.9682 & 11.9549 & 0.4212 & 0.0030 & 12.8164 & 10.6858 & 0.4307 & \textbf{0.0017} &  \textbf{8.8391} &  \textbf{9.0867} & \textbf{0.5076} \\
                                  & 336    & 0.0058 & 13.3578 & 14.6572 & 0.4243 & 0.0087 & 20.4895 & 23.7903 & 0.3579 & \textbf{0.0026} & \textbf{11.8682} &  \textbf{9.6758} & \textbf{0.5074} \\
                                  & 720    & 0.0068 & 18.5861 & 22.1432 & 0.4315 & 0.1534 & 28.6021 & 47.4488 & 0.3982 & \textbf{0.0029} & \textbf{17.1895} & \textbf{19.1942} & \textbf{0.5078} \\
%\multicolumn{2}{c|}{Count}                 & 2     & 1 & 2 & 0 & 0 & 0 & 0 & 0 & 8 & 9 & 8 & 10\\
\bottomrule
\end{tabular}}
\label{tab:nbeats}
\end{table*}



==> table/nsformer_experiment.tex <==
\begin{table*}[ht]
\centering
\caption{Detailed experimental results on six real-world datasets (four cases) with NSFormer.}
\resizebox{\columnwidth}{!}{\begin{tabular}{c|c|cccc|cccc}
\toprule
\multicolumn{2}{c|}{Methods} & \multicolumn{4}{c|}{NSFormer + MSE} & \multicolumn{4}{c}{NSFormer + TILDE-Q} \\
\midrule
\multicolumn{2}{c|}{Metric} & MSE & DTW & TDI & LCSS & MSE & DTW & TDI & LCSS \\
\midrule\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTh2}}
&  96 & 0.1868 ± 0.0173 & 5.7546 ± 0.5472  & 2.0024 ± 0.1875  & 0.5522 ± 0.0504 & \textbf{0.1629 ± 0.0083} & \textbf{5.1673 ± 0.0355}  & \textbf{1.4536 ± 0.5094}  & \textbf{0.6083 ± 0.0080} \\
& 192 & 0.2311 ± 0.0053 & 8.6408 ± 0.6911  & \textbf{3.8789 ± 0.0671}  & 0.5301 ± 0.0440 & \textbf{0.2016 ± 0.0056} & \textbf{8.0815 ± 0.0596}  & 4.0217 ± 0.1380  & \textbf{0.5963 ± 0.0004} \\
& 336 & \textbf{0.2624 ± 0.0167} & 11.1345 ± 0.3661 & \textbf{10.0050 ± 0.7225} & 0.5530 ± 0.0131 & 0.2760 ± 0.0136 & \textbf{11.0140 ± 0.0735} & 10.8131 ± 0.7981 & \textbf{0.5598 ± 0.0050} \\
& 720 & \textbf{0.2391 ± 0.0025} & 15.9557 ± 0.0797 & \textbf{18.2158 ± 1.4161} & 0.5409 ± 0.0154 & 0.2663 ± 0.0102 & \textbf{15.0010 ± 0.1701} & 19.5509 ± 1.3960 & \textbf{0.5575 ± 0.0084} \\
\midrule


\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTm2}}
&  96 & \textbf{0.0682 ± 0.0011} & \textbf{3.2222 ± 0.0710}  & \textbf{1.5062 ± 0.0636}  & \textbf{0.7681 ± 0.0029} & 0.0704 ± 0.0017 & 3.2704 ± 0.0382  & 1.5464 ± 0.0593  & 0.7678 ± 0.0018 \\
& 192 & \textbf{0.1107 ± 0.0061} & 5.6567 ± 0.1432  & 3.1250 ± 0.3309  & 0.6897 ± 0.0052 & 0.1142 ± 0.0097 & \textbf{5.4756 ± 0.0160}  & \textbf{3.0431 ± 0.1125}  & \textbf{0.7091 ± 0.0051} \\
& 336 & 0.1655 ± 0.0156 & 9.0536 ± 0.2199  & \textbf{7.3496 ± 0.2607}  & 0.6285 ± 0.0146 & \textbf{0.1590 ± 0.0033} & \textbf{8.9267 ± 0.1396}  & 8.5419 ± 0.8318  & \textbf{0.6450 ± 0.0049} \\
& 720 & 0.2349 ± 0.0202 & 14.8967 ± 0.3186 & \textbf{19.1985 ± 1.7474} & 0.5587 ± 0.0156 & \textbf{0.2209 ± 0.0126} & \textbf{14.8251 ± 0.0936} & 20.4820 ± 0.6624 & \textbf{0.5892 ± 0.0030} \\
\midrule


\multirow{4}{*}{\rotatebox[origin=c]{90}{ECL}}
&  96 & \textbf{0.3117 ± 0.0102} &  3.1460 ± 0.0466 & \textbf{0.3059 ± 0.0078} & 0.6839 ± 0.0051 & 0.3136 ± 0.0069 &  \textbf{3.0445 ± 0.0511} & 0.3170 ± 0.0273 & \textbf{0.6876 ± 0.0012} \\
& 192 & 0.3789 ± 0.0160 &  4.6092 ± 0.0077 & \textbf{0.3790 ± 0.0398} & 0.6736 ± 0.0252 & \textbf{0.3453 ± 0.0158} &  \textbf{4.4510 ± 0.1726} & 0.3892 ± 0.0469 & \textbf{0.6853 ± 0.0049} \\
& 336 & 0.3856 ± 0.0072 &  6.2827 ± 0.0620 & \textbf{0.2954 ± 0.0678} & 0.6724 ± 0.0098 & \textbf{0.3633 ± 0.0062} &  \textbf{6.0038 ± 0.0717} & 0.3573 ± 0.0336 & \textbf{0.6953 ± 0.0075} \\
& 720 & 0.4102 ± 0.0426 & 10.0263 ± 0.0869 & 1.7172 ± 1.0628 & 0.6680 ± 0.0107 & \textbf{0.3999 ± 0.0071} &  \textbf{9.6903 ± 0.0497} & \textbf{0.6640 ± 0.2962} & \textbf{0.6716 ± 0.0059} \\
\midrule

\multirow{4}{*}{\rotatebox[origin=c]{90}{Exchange}}
&  96 & 0.1514 ± 0.0505 & 8.4840 ± 0.1408  &  \textbf{6.2843 ± 0.3800}  & 0.4600 ± 0.0100 & \textbf{0.1078 ± 0.0084} & \textbf{8.0182 ± 0.2299}  &  7.4383 ± 0.6279  & \textbf{0.4667 ± 0.0037} \\
& 192 & 0.2514 ± 0.0280 & \textbf{10.7493 ± 0.8153} &  \textbf{14.7287 ± 2.0162} & 0.4723 ± 0.0105 & \textbf{0.2219 ± 0.0247} & 11.0704 ± 0.5110 &  15.5720 ± 3.1424 & \textbf{0.4898 ± 0.0191} \\
& 336 & 0.5246 ± 0.0908 & 12.3626 ± 1.0148 &  25.7294 ± 1.0591 & 0.4873 ± 0.0138 & \textbf{0.4219 ± 0.0740} & \textbf{11.9023 ± 0.5967} &  \textbf{23.2522 ± 1.5396} & \textbf{0.4928 ± 0.0049} \\
& 720 & 0.8866 ± 0.1059 & 18.8469 ± 3.5656 & 54.3978 ± 10.9369 & 0.5006 ± 0.0075 & \textbf{0.7557 ± 0.0535} & \textbf{13.7467 ± 1.3978} &  \textbf{42.9306 ± 9.0610} & \textbf{0.5199 ± 0.0201} \\
\midrule

\multirow{4}{*}{\rotatebox[origin=c]{90}{Traffic}}
&  96 & \textbf{0.1916 ± 0.0131} & 1.7903 ± 0.0393 & 0.0148 ± 0.0006 & 0.9012 ± 0.0076 & 0.2035 ± 0.0101 & \textbf{1.7658 ± 0.0213} & \textbf{0.0134 ± 0.0007} & \textbf{0.9088 ± 0.0069} \\
& 192 & \textbf{0.1829 ± 0.0086} & 2.7411 ± 0.0295 & 0.0083 ± 0.0001 & 0.9000 ± 0.0040 & 0.1838 ± 0.0113 & \textbf{2.7329 ± 0.0139} & \textbf{0.0079 ± 0.0002} & \textbf{0.9038 ± 0.0133} \\
& 336 & 0.2017 ± 0.0046 & 3.7920 ± 0.0107 & 0.0049 ± 0.0002 & 0.8959 ± 0.0021 & \textbf{0.1919 ± 0.0054} & \textbf{3.7476 ± 0.0310} & \textbf{0.0046 ± 0.0001} & \textbf{0.8993 ± 0.0019} \\
& 720 & 0.2294 ± 0.0077 & 6.0884 ± 0.1178 & 0.0027 ± 0.0001 & 0.8833 ± 0.0077 & \textbf{0.2287 ± 0.0071} & \textbf{5.8202 ± 0.0803} & \textbf{0.0024 ± 0.0001} & \textbf{0.8972 ± 0.0030} \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Weather}}
&  96 & 0.0017 ± 0.0005 &  8.2914 ± 1.1221 &  7.8379 ± 1.5827 & 0.4230 ± 0.0378 & \textbf{0.0012 ± 0.0001} &  \textbf{5.7786 ± 0.0468} &  \textbf{5.4118 ± 0.1960} & \textbf{0.5451 ± 0.0037} \\
& 192 & 0.0020 ± 0.0002 &  9.9842 ± 0.4992 & 10.8039 ± 1.9632 & 0.4536 ± 0.0025 & \textbf{0.0014 ± 0.0000} &  \textbf{7.3667 ± 0.0967} &  \textbf{6.2922 ± 0.2090} & \textbf{0.5532 ± 0.0060} \\
& 336 & 0.0018 ± 0.0002 & 13.6885 ± 0.7604 & 14.9242 ± 1.3217 & 0.4308 ± 0.0161 & \textbf{0.0015 ± 0.0001} &  \textbf{9.9883 ± 0.0800} &  \textbf{9.0103 ± 0.5340} & \textbf{0.5529 ± 0.0020} \\
& 720 & 0.0022 ± 0.0002 & 16.7372 ± 0.5878 & 33.7388 ± 4.4616 & 0.4751 ± 0.0025 & \textbf{0.0020 ± 0.0000} & \textbf{14.7109 ± 0.4148} & \textbf{17.1988 ± 0.9428} & \textbf{0.5405 ± 0.0051} \\
\bottomrule
\end{tabular}}
\end{table*}
